DifFUSER: Diffusion Model for Robust Multi-Sensor Fusion in 3D Object Detection and BEV Segmentation

Diffusion models have recently gained prominence as powerful deep generative models, demonstrating unmatched performance across various domains. However, their potential in multi-sensor fusion remains largely unexplored. In this work, we introduce DifFUSER, a novel approach that leverages diffusion models for multi-modal fusion in 3D object detection and BEV map segmentation. Benefiting from the inherent denoising property of diffusion, DifFUSER is able to refine or even synthesize sensor features in case of sensor malfunction, thereby improving the quality of the fused output. In terms of architecture, our DifFUSER blocks are chained together in a hierarchical BiFPN fashion, termed cMini-BiFPN, offering an alternative architecture for latent diffusion. We further introduce a Gated Self-conditioned Modulated (GSM) latent diffusion module together with a Progressive Sensor Dropout Training (PSDT) paradigm, designed to add stronger conditioning to the diffusion process and robustness to sensor failures. Our extensive evaluations on the Nuscenes dataset reveal that DifFUSER not only achieves state-of-the-art performance with a 70.04% mIOU in BEV map segmentation tasks but also competes effectively with leading transformer-based fusion techniques in 3D object detection.

==> figs/0_thumbnail.tex <==
%\begin{figure*}
%\noindent\includegraphics[width=\linewidth]{imgs/thumbnail}
%\captionof{figure}{We propose to formulate multi-modal fusion as a denoising diffusion process
%from noisy to refined BEV features, which are then fed into task-specific heads for 3D object detection and BEV map segmentation.}
%\label{fig:thumbnail}
%\end{figure*}%


==> figs/5_sensor_drop.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/sensor_drop.pdf}
    \caption{Performance Comparison of DifFUSER with \n and without Sensor Drop (either Lidar or Camera)}
    \label{fig:sensor_drop}
    \vspace{-1.5em}
\end{figure}


==> sec/3_premilinaries.tex <==
\section{Premilinaries}
% It's essential to understand the foundational concepts that our work builds upon, particularly Diffusion Probabilistic Models (DPMs). These models, underpinning the one of the core components in our methodology, are instrumental in driving the performance and capabilities of DifFUSER

\textbf{Revisit Diffusion Probabilistic Models}.
For diffusion probabilistic models \cite{diffusion,diffbeatsgan}, such as DDPM \cite{ddpm} and DDIM \cite{ddim}, the training involves a forward noising process and a reverse denoising process. In the forward noising process, Gaussian noise $\varepsilon$ is gradually added to the real sample $x_0$ via a discrete \textit{stochastic differential equation} (SDE):
\[q(x_t, x_0) = \sqrt{\bar{\alpha_t}}x_0 + \varepsilon \sqrt{1 - \bar{\alpha_t}},\]
where $\bar{\alpha_t}$ is a hyperparameters and $\varepsilon \sim \mathcal{N}(0, I)$. If the time step $t$ is large, $x_t$ would become Gaussian noise.
The diffusion model is trained to reverse the noising process $p_{\theta}((x_{t-1}|x_t) = \mathcal{N}(\mu_{\theta}(x_t), \sigma_{\theta}(x_t))$, where $\mu_{\theta}(x_t)$ and $\sigma_{\theta}(x_t)$ are the predicted mean and standard deviation of the Gaussian distribution. The training objective is to minimize the variational lower bound (VLB) of the log-likelihood of the real sample $x_0$:
\begin{align}
    % L_{vlb} = & - \log p_0(x_0 | x_1) \nonumber \\
    %           & + \sum_t D_{KL}(q(x_t | x_1, x_0) || p_{\theta}(x_t-1 | x_t,x_0)).
    L_{vlb} = & - p_0(x_0 | x_1) \nonumber \\
              & + \sum_t D_{KL}(q(x_t | x_1, x_0) || p_{\theta}(x_t-1 | x_t,x_0)).
\end{align}
Where $p_0(x_0 | x_1)$ is the distribution of $x_0$ given $x_1$, and $D_{KL}$ is the Kullback-Leibler divergence.

\input{figs/2_architecture}




\noindent\textbf{Faster Sampling.} The reverse denoising process is a discrete SDE that gradually maps a Gaussian noise into a sample. At each time step, given $x_t$, it predicts the next reverse step:
\[
    p^{\left( t \right)}(x_{t-1} | x_t, x_0) =
    \begin{cases}
        \mathcal{N}\left( p^{\left( 1 \right)}_\theta(x_1, x_0), \sigma^2I \right) & \text{if } t = 1 \\
        q(x_{t-1} | x_t, p^{\left( t \right)}_\theta(x_t,x_0)) & \text{otherwise.}
    \end{cases}
\]
Given that fast inference is an important factor in real-world applications, DDPM sampler \cite{ddpm} is not considered a practical model due to its slow sampling speed. Later, we explore and compare the potential of using training-free faster diffusion samplers, such as the first-order sampler DDIM \cite{ddim}, or higher-order samplers like DPM-Solver++ \cite{dpmsolver++} and DEIS \cite{deis}.


